Deformable ProtoPNet: An Interpretable Image Classifier Using Deformable Prototypes

We present a deformable prototypical part network (Deformable ProtoPNet), an interpretable image classifier that integrates the power of deep learning and the interpretability of case-based reasoning. This model classifies input images by comparing them with prototypes learned during training, yielding explanations in the form of "this looks like that." However, while previous methods use spatially rigid prototypes, we address this shortcoming by proposing spatially flexible prototypes. Each prototype is made up of several prototypical parts that adaptively change their relative spatial positions depending on the input image. Consequently, a Deformable ProtoPNet can explicitly capture pose variations and context, improving both model accuracy and the richness of explanations provided. Compared to other case-based interpretable models using prototypes, our approach achieves state-of-the-art accuracy and gives an explanation with greater context. The code is available at https://github.com/jdonnelly36/Deformable-ProtoPNet.

==> methodology.tex <==
% Methodology
\section{Methodology}

In this section, we introduce the concept of deformable prototypes, before describing the architecture and training algorithm of Deformable ProtoPNet.

\subsection{Deformable Prototypes}
% What are prototypes in general?
% What is different about deformable prototypes?
% Will introduce, deformation, similarity score here
Previous work such as \cite{ProtoPNet, originalProtoPNet, ProtoTree, TesNet} has introduced the idea of latent space prototypes using a convolution-like procedure of scanning over a regular grid. Deformable prototypes differ from this approach because they are composed of multiple prototypical parts that are allowed change their spatial locations. Figure \ref{fig.deformation_intro} demonstrates this idea at a conceptual level; the parts are no longer constrained to a simple grid pattern, and as such can explicitly capture spatial variations. 

In this work, we use $\mathbf{\hat{p}}^{(c, l)}$ to denote the $l$th prototype of class $c$, and use $\mathbf{\hat{p}}^{(c, l)}_{m, n}$ to denote the $(m, n)$th prototypical part. We use spatial indices $(m,n)$ to represent the location of each part in the prototypes. 

We restrict that each prototypical part is a unit vector representing some point on a hypersphere

% Talk about how deformation is done, introduce square -- deform -- sqrt procedure
% How to get offset, how to apply offset and interpolate
% Similarity metric
% Introduce margin and orthogonality loss here
% Also talk about implementation here - i.e., normalization, zero vector, 

\subsection{Architecture}

\subsection{Training}
% prototype projection needs to be discussed (it's different from before)

\subsection{Prototype visualization}


\section{Methods}
\label{sec:methods}
%Explain benefits of original ProtoP in intro; benefits of our improvements
% 
% For now, I introduce notation here in a list to simplify writing
% Start straight in on deformable prototypes, will need a figure to show what deformations are 
% c = class of the prototype
% l = the lth prototype in class c
% m, n = position of component within prototype
%    - include that we can account for dilation
% p^ = the unit vector prototype
% z^ = the unit vector latent input
% a,b = poisiton in the latent input
%delta takes as input: z^, m, n, a, b and produces as output Delta_1, Delta_2

In the following sections, we first introduce the specific concepts necessary to understand Deformable ProtoPNet, followed by architecture and training details.
%$f$ -- The backbone convolutional network
%$g$ -- The prototype application layer
%$h$ -- The offset prediction branch
%$\mathbf{I}$ -- The input tensor
%$\mathbf{O}$ -- The offset tensor

\subsection{Distance Metric}
\label{sec:methods:distance_metric}
The activation of each prototype in Deformable ProtoPNet is computed using an angle based distance metric on the unit hypersphere, which we find easier to train than l2 distance based metrics. Our implementation is detailed below.

Recall that, for two vectors $\mathbf{a}, \mathbf{b}$, the dot product between these vectors follows $\frac{\mathbf{a} \cdot \mathbf{b}}{\|a\| \|b\|} = \cos(\theta)$, where $\theta$ is the angle between the two vectors in radians. We use this angle to measure the distance between prototype vectors and patches of the latent space and $\cos(\theta)$ as a corresponding activation metric, interpreting a high value for $\cos(\theta)$ as a high similarity between a prototype and latent patch.

Inspired by \cite{arc_face}, we leverage this metric to introduce an additive margin loss in order to encourage prototypes and patches of their own class to match closely. Specifically, we define:
\begin{equation}
\label{eqn.additive_marging}
    g(\mathbf{X}_{\text{latent}})^{(k)}_{i,j} = 
    \begin{cases}
    \cos(\theta + m) &\text{if } k \in \text{class}(\mathbf{X})\\
    \cos(\theta) & \text{else},
    \end{cases}
\end{equation}
where $\theta=\arccos(\frac{\mathbf{p}^{(k)} \cdot \mathbf{x}_{i,j}}{\|\mathbf{p}^{(k)}\|\|\mathbf{x}_{i,j}\|})$.

For prototypes of an arbitrary spatial dimension $s_1 \times s_2$ with channel length $c$, we stack each component to for a vector $\mathbf{p}^(k)\in \mathbb{R}^{s_1 * s_2 * c}$. The angle between this prototype and the corresponding stacked latent patch $\mathbf{x}$ is then computed similarly as $\cos(\theta) = \frac{\mathbf{p}^{(k)} \cdot \mathbf{x}_{i,j}}{\|\mathbf{p}^(k)\| \|\mathbf{x}_{i,j}\|\sqrt{s_1s_2}}$. This stacked dot product is equivalent to convolving the unstacked prototype over the target patch, and is computed as such.

Note that this introduces a problem: if $\|\mathbf{p}^{(k)}\|=0$ or $\|\mathbf{x}_{i,j}\|=0$, the quotient used to compute $\theta$ is undefined. 

\subsection{Deformable prototypes}
\label{sec:methods:deformable_prototypes}

The primary innovation of this work comes from the introduction of deformable prototypes. Informally, the prototypes of Deformable ProtoPNet change their shape and orientation at prediction time based on the input image. 

For simplicity, consider a single prototype $\mathbf{p}^{(k)}$ composed of size $s_1 * s_2$ applied with no margin, and let $\mathbf{X} = f(\mathbf{X})$ for the duration of this subsection. Normally this prototype is used to compute an activation map $g(\mathbf{X})^{(k)}$ from a latent image representation $\mathbf{X}$ according to:
\begin{equation}
\label{eqn.normal_prototypes}
    g(\mathbf{X})^{(k)}_{i,j} = \sum_m^{s_1} \sum_n^{s_2} \frac{\mathbf{p}^{(k)}_{m,n} \cdot \mathbf{x}_{i+m, j+n}}{\|\mathbf{p}^{(k)}_{m,n}\|\|\mathbf{x}_{i+m, j+n}\|\sqrt{s_1s_2}}
\end{equation}

In this structure, each component of $\mathbf{p}$ is applied on a regular grid. Drawing from \cite{deformable_convolution}, Deformable ProtoPNet introduces offsets $\delta(\mathbf{X})$ which define where each component of the prototype is applied. We generalize \ref{eqn.normal_prototypes} by using these offsets, allowing each piece of a prototype to move differently for each input image and each center location $i,j$. Specifically, we compute:
\begin{equation}
\label{eqn.deformation}
    g(\mathbf{X})_{i,j} = \sum_m^{s_1} \sum_n^{s_2} \frac{\mathbf{p}_{m,n}\cdot \mathbf{x}_{\Delta_1, \Delta_2}}{\|\mathbf{p}_{m,n}\|\|\mathbf{x}_{\Delta_1, \Delta_2}\|\sqrt{s_1s_2}}
\end{equation}
where $\Delta_1 = i + m + \delta(\mathbf{x}_{i+m,j+n})_1$ and $\Delta_2 = i + m + \delta(\mathbf{x}_{i+m,j+n})_2$ denote a fractional location in $\mathbf{X}$, as offsets are most often fractional. We compute fractional locations via bilinear interpolation between the four grid locations. For further implementation details, see the supplement \textbf{In the supplement, we may want to include why we need to do the square - deform - sqrt procedure}.
%More rigorously, Deformable ProtoPNet integrates deformable convolution, as defined in \cite{deformable_convolution}, by introducing a secondary branch to the embedding network. This branch consists of a convolutional neural network $h: f(\mathbf{I}) \rightarrow \mathbf{O}$, where $\mathbf{O}$ is a tensor of offsets containing an $(x, y)$ pair of offsets for each piece of each prototype at each location in $f(\mathbf{I})$. 
% This notation is terrible - way too much subscript. Need to figure something else out

\subsection{Orthogonality Loss}
\label{sec:methods:orthogonality_loss}
The introduction of deformations creates a problem: what if all pieces %of a prototype learn a single concept? Because of the introduction of %deformations, each piece of a given prototype is able to collapse to %look for the same concept. We aim to address this problem by encouraging %keypoints within a prototype to be orthogonal to one another. We do so %by introducing a new loss term inspired by \cite{Tesnet}: orthogonality %loss.

Define the matrix $\mathbf{O}^{(k)}=\begin{bmatrix}
\mathbf{p}^{(k)}_{0,0} & \mathbf{p}^{(k)}_{1,0} &\hdots & \mathbf{p}^{(k)}_{s_1,0} & \mathbf{p}^{(k)}_{0,1} & \mathbf{p}^{(k)}_{1,1} & \hdots & \mathbf{p}^{(k)}_{s_1,s_2}
\end{bmatrix}$. With this keypoint matrix, we define inter-keypoint orthogonality loss across $k$ prototypes as follows:
\begin{equation}
\label{eqn.ortho_loss}
    l_{ortho} = \sum_{k=1}^K \|\mathbf{O}^{(k)}\mathbf{O}^{(k)T} - \mathbf{I}\|^2_F
\end{equation}
This loss term discourages keypoints within a prototype form being nearby within the latent space, and thereby encourages them to learn distinct concepts.


\subsection{Architecture}
\label{sec:methods:architecture}
At a high level, Deformable ProtoPNet uses an architecture similar to that of other case-based reasoning models such as \cite{ProtoPNet}. Any network input $\mathbf{X}$ is first fed through a backbone convolutional network, denoted as $f$. $f(\mathbf{X}$ is passed through an offset prediction network $\delta(f(\mathbf{X}))$, which is used to compute the output of prototype application layer $g$ as described in \ref{sec:methods:deformable_prototypes}. Finally, $g(f(\mathbf{X}), \delta(f(\mathbf{x})))$ passes through a final fully connected layer $h$ to produce logits for each class. The maximum logit is taken to be the class prediction. 

In more detail, the backbone convolutional network may be any architecture; for this work, we experiment with VGG16, VGG19, Densenet121, Densenet161, Resnet34, and Resnet50 \cite{vgg, densenet, resnet}. This backbone network produces a useful feature embedding space $f(\mathbf{X})$, which is input into the prototype layer $g$ and the offset prediction branch $\delta$.

For a given input $\mathbf{X}$, we compute a set of offsets $\delta(f(\mathbf{X}))$ by passing the latent representation of input $\mathbf{X}$ into a secondary convolutional branch $\delta$. A distinct offset in the row and column dimension is computed for each component of each prototype at each applied location in the latent space. That is, for a network with $k$ prototypes consisting of $s_x\times s_y$ components and a latent space of size $l_x,l_y$, $\delta$ will produce $2 \times k \times s_x \times s_y \times l_x \times l_y$ distinct offsets assuming same padding, unit stride, and dilation of 1 are used.

The latent representation and offsets are then fed into the prototype layer $g$, which computes activation values for each prototype at each center location. In this computation, the pieces of each prototype move according to the predicted offsets, and compute an activation according to \ref{eqn.additive_marging} at their new interpolated location. This yields a prototype activation map $\mathbf{A}^{(k)} = g(f(\mathbf{X}); \delta(f(\mathbf{X})))^{(k)}$ for each prototype. The global maximum of $\mathbf{A}^{(k)}$ is then taken, producing a single activation score for each prototype in the network.

Finally, these activation scores are fed into a fully connected layer $h$ to produce an output logit for each class. The maximum such logit is taken to be the final class prediction.

\subsection{Training Regime}
\label{sec:methods:training_regime}
Similar to \cite{ProtoPNet}, we split training into three major phases: 1) stochastic gradient descent (SGD) of parameters before the last layer, 2) projection of prototypes, and 3) optimization of the last layer.

The majority of training time is dedicated to the first phase of training. In this phase, we attempt to learn a useful feature embedding space, set of prototypes, and offset prediction branch. We use cross entropy loss (CrsEnt) to encourage accuracy, additive margin loss to encourage prototypes to cluster close to features of their class, and l2 loss on the predicted offsets to discourage overfitting. This gives us the following optimization problem:
\begin{equation}
\label{eqn.loss}
    \min_{\mathbf{P}, w_{\text{conv}}, w_{\delta}} \frac{1}{N} \sum_{n=1}^N \text{CrsEnt}(h \circ g(f(\mathbf{X}^{(n)}); \delta \circ f(\mathbf{X}^{(n)}))) + \lambda l(\mathbf{X}^{(n)})
\end{equation}
where $w_{\text{conv}}$ denotes the parameters of the backbone convolutional network, $w_{\delta}$ denotes the parameters of the offset prediction branch, and $l$ is l2 loss on the predicted offset, ie:
\begin{equation}
\label{eqn.l2_loss}
    l(\mathbf{X}) = \|\delta \circ f(\mathbf{X}))\|_2
\end{equation}
We use SGD to optimize over this problem. Empirically, we find that splitting this phase into three sections improves training in some settings. Specifically, we first train only the embedding CNN $f$, followed by the embedding CNN $f$ and prototypes $\mathbf{P}$ without deformation, and finally $f$, $\mathbf{P}$, and $\delta$ together. This allows the pieces of each prototype to take on some meaning prior to being able to move, encouraging them to learn distinct concepts. 

In order to ensure interpretability, it is important that each prototype component match some patch of a training image exactly. This ensures that each prototype can be depicted using the corresponding patch of a training image, enabling a faithful explanation of what the network 'looks for'. We achieve this goal by projecting the pieces of each prototype onto the latent patches of the training image that produced the best activation for that prototype. That is, we update each component $c$ of each prototype $k$ according to:
% I don't think this makes much sense right now
\begin{equation}
\label{eqn.projection}
    \mathbf{p}^{(k)}_c \leftarrow \mathbf{z}_{\Delta_1, \Delta_2}  \text{ where } \mathbf{z} = \max_{\mathbf{X},i,j}(g(f(\mathbf{X}))_{i,j}
\end{equation}

Finally, after projection we fix all other model parameters and optimize only the last layer connections. 

\section{Results and Discussion}
\label{sec:results+discussion}
% experiment list: https://docs.google.com/document/d/1lnVXnFu-g7xRioCJcjpuBAA7dILNJoKNDvGgzxBCmyE/edit?usp=sharing 

% Use a pacmap to demonstrate improved cluster structure of deformable ProtoP?
% Also include graph demonstrating higher percentage of nearest neighbors are of wrong class in l2-distance

% I'm going to stard dropping in results as they come
\begin{table*}
    \begin{tabular}{|l|l|l||l|}
    \hline
    Margin & Orthogonality Loss & Deformation & Accuracy\\ \hline
    0 & 0 & True & 83.95\\ \hline
    0 & 0 & False & 83.45\\ \hline
    0 & 0.005 & True & 84.26\\ \hline
    0 & 0.005 & False & 84.05\\ \hline
    \textbf{0.4} & \textbf{0} & \textbf{True} & \textbf{85.35}\\ \hline
    0.4 & 0 & False & 83.64\\ \hline
    0.4 & 0.005 & True & 81.86\\ \hline
    0.4 & 0.005 & False & 82.82\\ \hline
    \end{tabular}
\end{table*}

%some comparison tables
\begin{table*}
    \centering
    \begin{tabular}{|l|l|l||l|l|l|}
    \hline
    Base & ProtoPNet & Baseline & Base & ProtoPNet & Baseline \\ \hline
    VGG16 & 76.1 $\pm$ 0.2  & 74.6 $\pm$ 0.2 & VGG19 & 78.0 $\pm$ 0.2 & 75.1 $\pm$ 0.4 \\ \hline
    Res34 & 79.2 $\pm$ 0.1 & 82.3 $\pm$ 0.3 & Res152 & 78.0 $\pm$ 0.3 & 81.5 $\pm$ 0.4
    \\ \hline
    Dense121 & 80.2 $\pm$ 0.2 & 80.5 $\pm$ 0.1 & Dense161 & 80.1 $\pm$ 0.3 & 82.2 $\pm$ 0.2
    \\ \hline
    \end{tabular}
    \begin{tabular}{|l|l|}
    \hline
    Interpretability & Model: accuracy                      
    
    \\ \hline
    None & \textbf{B-CNN}: 85.1 (bb), 84.1 (full)                                         
    \\ \hline
    \begin{tabular}[c]{@{}l@{}}Object-level attn.\end{tabular}                                & \textbf{CAM}: 70.5 (bb), 63.0 (full)  \\ \hline
    
    \begin{tabular}[c]{@{}l@{}}Part-level\\ attention \end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}} \textbf{Part R-CNN}: 76.4 (bb+anno.); \textbf{PS-CNN}: 76.2 (bb+anno.);\\
    \textbf{PN-CNN}: 85.4 (bb+anno.); \textbf{DeepLAC}: 80.3 (anno.);\\ \textbf{SPDA-CNN}: 85.1 (bb+anno.); \textbf{PA-CNN}: 82.8 (bb);\\ \textbf{MG-CNN}: 83.0 (bb), 81.7 (full); \textbf{ST-CNN}: 84.1 (full);\\ \textbf{2-level attn.}: 77.9 (full); \textbf{FCAN}: 82.0 (full);\\ \textbf{Neural const.}: 81.0 (full); \textbf{MA-CNN}: 86.5 (full);\\ \textbf{RA-CNN}: 85.3 (full)\end{tabular} \\ \hline
    
    \begin{tabular}[c]{@{}l@{}}Part-level attn. +\\ prototypical cases\end{tabular} &
    
    \begin{tabular}[c]{@{}l@{}} \textbf{ProtoPNet} (ours):\\ 
                               80.8 (full, VGG19+Dense121+Dense161-based)  \\
                               84.8 (bb, VGG19+ResNet34+DenseNet121-based)
    \end{tabular}
    
    %\begin{tabular}[c]{@{}l@{}}\textbf{ProtoPNet} (ours): 84.8 (bb, VGG19+ResNet34+DenseNet121-based)\end{tabular}
    
    %ProtoPNet (ours): 84.8 (bb, VGG19+ResNet34+DenseNet121-based)
    
    \\ \hline
    \end{tabular}
\end{table*}
\section{Conclusion}
\label{sec:conclusion}
